On normalization-equivariance properties of supervised and unsupervised denoising methods: a survey

Image denoising is probably the oldest and still one of the most active research topic in image processing. Many methodological concepts have been introduced in the past decades and have improved performances significantly in recent years, especially with the emergence of convolutional neural networks and supervised deep learning. In this paper, we propose a survey of guided tour of supervised and unsupervised learning methods for image denoising, classifying the main principles elaborated during this evolution, with a particular concern given to recent developments in supervised learning. It is conceived as a tutorial organizing in a comprehensive framework current approaches. We give insights on the rationales and limitations of the most performant methods in the literature, and we highlight the common features between many of them. Finally, we focus on on the normalization equivariance properties that is surprisingly not guaranteed with most of supervised methods. It is of paramount importance that intensity shifting or scaling applied to the input image results in a corresponding change in the denoiser output.

==> aux.tex <==
\relax 
\citation{photon_noise}
\citation{DND}
\citation{unprocessing}
\citation{cycleisp}
\citation{poisson_estimation}
\citation{Anscombe}
\citation{Starck98}
\citation{BoulangerTMI2010}
\citation{MakitaloTIP2011}
\citation{ReviewElad2023}
\providecommand \oddpage@label [2]{}
\@writefile{toc}{\contentsline {section}{\numberline {I}Introduction}{1}\protected@file@percent }
\newlabel{pgnoise_intro}{{1}{1}}
\newlabel{awgn_intro}{{2}{1}}
\citation{unprocessing}
\citation{cycleisp}
\citation{PNGAN}
\citation{scunet}
\citation{fully_synthetic_training}
\newlabel{PSNRcpu}{{I}{2}}
\@writefile{lof}{\contentsline {figure}{\numberline {1}{\ignorespaces Execution time on CPU for images of size $512\times 512$ v.s the average PSNR results on the union of Set12 and BSD68 datasets for Gaussian noise with $\sigma =25$ for popular methods.}}{2}\protected@file@percent }
\@writefile{toc}{\contentsline {section}{\numberline {II}Review of supervised learning methods}{2}\protected@file@percent }
\@writefile{toc}{\contentsline {subsection}{\numberline {\unhbox \voidb@x \hbox {II-A}}Principle of supervised learning}{2}\protected@file@percent }
\newlabel{principle_of_supervised_learning}{{\unhbox \voidb@x \hbox {II-A}}{2}}
\newlabel{f_risk}{{3}{2}}
\newlabel{f_opt}{{4}{2}}
\newlabel{theta_opt}{{5}{2}}
\newlabel{f_risk_emp}{{6}{2}}
\citation{mlp_inventor}
\citation{mlp}
\citation{mlp_universal1}
\citation{mlp_universal2}
\citation{mlp_universal3}
\citation{mlp}
\citation{mlp}
\citation{dset_labelme}
\citation{berkeley}
\@writefile{toc}{\contentsline {subsection}{\numberline {\unhbox \voidb@x \hbox {II-B}}Classes of parameterized functions}{3}\protected@file@percent }
\@writefile{toc}{\contentsline {subsubsection}{\numberline {\unhbox \voidb@x \hbox {II-B}1}Multi-layer perceptron (MLP)}{3}\protected@file@percent }
\@writefile{toc}{\contentsline {paragraph}{\numberline {\unhbox \voidb@x \hbox {II-B}1a}Mathematical description}{3}\protected@file@percent }
\newlabel{mlp_equation}{{7}{3}}
\newlabel{tanh}{{9}{3}}
\newlabel{relu}{{10}{3}}
\@writefile{toc}{\contentsline {paragraph}{\numberline {\unhbox \voidb@x \hbox {II-B}1b}MLP applied on patches for image denoising}{3}\protected@file@percent }
\newlabel{mlp_burger_equation}{{11}{3}}
\citation{mlp}
\citation{BM3D}
\citation{normalization_morel}
\citation{tnrd}
\citation{red30}
\citation{drunet}
\citation{dncnn}
\citation{ffdnet}
\citation{ircnn}
\citation{mwcnn}
\citation{ridnet}
\citation{dilated}
\citation{resnet}
\citation{unet}
\newlabel{CNN_section}{{\unhbox \voidb@x \hbox {II-B}2}{4}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {\unhbox \voidb@x \hbox {II-B}2}Convolutional neural networks (CNN)}{4}\protected@file@percent }
\@writefile{toc}{\contentsline {paragraph}{\numberline {\unhbox \voidb@x \hbox {II-B}2a}Mathematical description}{4}\protected@file@percent }
\newlabel{conv_equation}{{12}{4}}
\@writefile{lof}{\contentsline {figure}{\numberline {2}{\ignorespaces Standard 2D convolution}}{4}\protected@file@percent }
\newlabel{figure_conv2d}{{2}{4}}
\newlabel{cnn_equation}{{13}{4}}
\@writefile{toc}{\contentsline {paragraph}{\numberline {\unhbox \voidb@x \hbox {II-B}2b}Receptive field}{4}\protected@file@percent }
\citation{dncnn}
\citation{dncnn}
\citation{resnet}
\citation{batchnorm}
\citation{mlp}
\citation{dncnn}
\citation{berkeley}
\citation{jpeg_deblocking}
\citation{unet}
\citation{resnet}
\citation{drunet}
\citation{unet}
\citation{resnet}
\citation{drunet}
\citation{drunet}
\citation{dncnn}
\citation{unet}
\citation{resnet}
\citation{pixelshuffle}
\citation{dncnn}
\citation{dncnn}
\citation{ircnn}
\citation{ffdnet}
\citation{dncnn}
\@writefile{lof}{\contentsline {figure}{\numberline {3}{\ignorespaces The architecture of DnCNN denoising network}}{5}\protected@file@percent }
\newlabel{figure_dncnn}{{3}{5}}
\@writefile{toc}{\contentsline {paragraph}{\numberline {\unhbox \voidb@x \hbox {II-B}2c}Focus on DnCNN architecture}{5}\protected@file@percent }
\newlabel{dncnn_equation}{{16}{5}}
\@writefile{lof}{\contentsline {figure}{\numberline {4}{\ignorespaces The architecture of DRUNet denoising network}}{5}\protected@file@percent }
\newlabel{figure_drunet}{{4}{5}}
\@writefile{toc}{\contentsline {paragraph}{\numberline {\unhbox \voidb@x \hbox {II-B}2d}Focus on DRUNet architecture}{5}\protected@file@percent }
\citation{berkeley}
\citation{dset_waterloo}
\citation{dset_div2k}
\citation{dset_flickr2k}
\citation{attention}
\citation{n3net}
\citation{nlrn}
\citation{rnan}
\citation{swinir}
\citation{restormer}
\citation{scunet}
\citation{transformer_eccv}
\citation{nlmeans}
\citation{nlrn}
\citation{nlmeans}
\citation{nlmeans2}
\citation{nlmeans3}
\citation{nlmeans_parameters}
\citation{nlrn}
\citation{swinir}
\citation{restormer}
\citation{scunet}
\citation{n3net}
\citation{nlrn}
\citation{rnan}
\citation{swinir}
\citation{restormer}
\citation{scunet}
\citation{scunet}
\citation{scunet}
\citation{scunet}
\citation{drunet}
\citation{swinir}
\citation{attention}
\citation{swin}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {\unhbox \voidb@x \hbox {II-B}3}Transformers}{6}\protected@file@percent }
\@writefile{toc}{\contentsline {paragraph}{\numberline {\unhbox \voidb@x \hbox {II-B}3a}Mathematical description}{6}\protected@file@percent }
\newlabel{attention_eq}{{16}{6}}
\newlabel{attention2}{{17}{6}}
\@writefile{lof}{\contentsline {figure}{\numberline {5}{\ignorespaces The architecture of SCUNet denoising network}}{6}\protected@file@percent }
\newlabel{figure_scunet}{{5}{6}}
\@writefile{toc}{\contentsline {paragraph}{\numberline {\unhbox \voidb@x \hbox {II-B}3b}Focus on SCUNet architecture}{6}\protected@file@percent }
\citation{drunet}
\citation{drunet}
\citation{scunet}
\citation{dncnn}
\citation{ridnet}
\citation{mlp}
\citation{drunet}
\citation{mwcnn}
\citation{tnrd}
\citation{scunet}
\citation{dncnn}
\citation{ridnet}
\citation{mlp}
\citation{drunet}
\citation{mwcnn}
\citation{tnrd}
\citation{scunet}
\citation{drunet}
\citation{pytorch}
\citation{sgd}
\citation{adam}
\citation{sgd}
\citation{dncnn}
\citation{drunet}
\citation{scunet}
\citation{ffdnet}
\citation{n3net}
\citation{nlrn}
\citation{sgd}
\@writefile{lof}{\contentsline {figure}{\numberline {6}{\ignorespaces Performance evolution of models with the number of parameters and execution time}}{7}\protected@file@percent }
\newlabel{graph}{{6}{7}}
\@writefile{toc}{\contentsline {subsection}{\numberline {\unhbox \voidb@x \hbox {II-C}}Parameter optimization}{7}\protected@file@percent }
\@writefile{toc}{\contentsline {subsubsection}{\numberline {\unhbox \voidb@x \hbox {II-C}1}Back-propagation}{7}\protected@file@percent }
\@writefile{toc}{\contentsline {subsubsection}{\numberline {\unhbox \voidb@x \hbox {II-C}2}Stochastic gradient descent}{7}\protected@file@percent }
\newlabel{batch}{{17}{7}}
\@writefile{loa}{\contentsline {algorithm}{\numberline {1}{\ignorespaces Stochastic Gradient Descent (SGD) algorithm}}{7}\protected@file@percent }
\newlabel{algo_sgd}{{1}{7}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {\unhbox \voidb@x \hbox {II-C}3}Adam optimization algorithm}{7}\protected@file@percent }
\citation{noise2noise}
\citation{noise2noise_improved}
\@writefile{loa}{\contentsline {algorithm}{\numberline {2}{\ignorespaces Adam algorithm}}{8}\protected@file@percent }
\newlabel{algo_adam}{{2}{8}}
\@writefile{toc}{\contentsline {subsection}{\numberline {\unhbox \voidb@x \hbox {II-D}}Weakly supervised learning}{8}\protected@file@percent }
\@writefile{toc}{\contentsline {subsubsection}{\numberline {\unhbox \voidb@x \hbox {II-D}1}Learning from noisy image pairs}{8}\protected@file@percent }
\newlabel{noise2noise_intro}{{18}{8}}
\newlabel{noise2noise}{{18}{8}}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {\unhbox \voidb@x \hbox {II-D}2}Learning from single noisy images}{8}\protected@file@percent }
\citation{SURE}
\citation{sure_loss}
\citation{SURE}
\citation{monte_carlo_sure}
\citation{sure_loss}
\citation{N2S}
\citation{N2V}
\citation{N2S}
\citation{N2K}
\citation{N2V}
\citation{N2S}
\citation{N2S}
\citation{pN2V}
\citation{laine}
\citation{convallaria}
\citation{N2S}
\@writefile{toc}{\contentsline {paragraph}{\numberline {\unhbox \voidb@x \hbox {II-D}2a}SURE}{9}\protected@file@percent }
\newlabel{sure_loss_}{{19}{9}}
\@writefile{toc}{\contentsline {paragraph}{\numberline {\unhbox \voidb@x \hbox {II-D}2b}Blind-spot networks}{9}\protected@file@percent }
\newlabel{noise2self_intro}{{\unhbox \voidb@x \hbox {II-D}2b}{9}}
\newlabel{noise2self}{{21}{9}}
\@writefile{toc}{\contentsline {paragraph}{\numberline {\unhbox \voidb@x \hbox {II-D}2c}Probabilistic blind-spot networks}{9}\protected@file@percent }
\citation{pN2V}
\citation{laine}
\citation{laine}
\citation{adam}
\citation{laine}
\citation{pN2V}
\citation{noisier2noise}
\citation{R2R}
\citation{noisier2noise}
\citation{R2R}
\citation{noise2noise}
\citation{R2R}
\citation{noise2score}
\citation{tweedie}
\citation{score_approx}
\citation{noise2score}
\@writefile{toc}{\contentsline {paragraph}{\numberline {\unhbox \voidb@x \hbox {II-D}2d}Noisier2Noise}{10}\protected@file@percent }
\newlabel{riskNr2N2}{{26}{10}}
\@writefile{toc}{\contentsline {paragraph}{\numberline {\unhbox \voidb@x \hbox {II-D}2e}Noise2Score}{10}\protected@file@percent }
\newlabel{tweedie_formula}{{29}{10}}
\citation{R2R}
\citation{noise2score}
\citation{noise2noise}
\citation{convallaria}
\citation{N2S}
\citation{N2V}
\citation{sure_loss}
\citation{pN2V}
\citation{laine}
\citation{noisier2noise}
\citation{R2R}
\citation{noise2score}
\citation{DND}
\citation{unprocessing}
\citation{cycleisp}
\citation{PNGAN}
\citation{scunet}
\citation{CARE}
\citation{canny}
\citation{bilateral}
\citation{nlmeans}
\citation{OWF}
\citation{yaroslavsky}
\citation{averaging_filters}
\citation{these}
\citation{bilateral}
\citation{nlmeans}
\citation{OWF}
\citation{bilateral}
\citation{nlmeans}
\newlabel{training_noise2score}{{30}{11}}
\@writefile{toc}{\contentsline {subsection}{\numberline {\unhbox \voidb@x \hbox {II-E}}Discussion and conclusion}{11}\protected@file@percent }
\@writefile{toc}{\contentsline {section}{\numberline {III}Unsupervised denoising methods}{11}\protected@file@percent }
\@writefile{toc}{\contentsline {subsection}{\numberline {\unhbox \voidb@x \hbox {III-A}}Weighted averaging methods}{11}\protected@file@percent }
\newlabel{nlm_weights}{{33}{11}}
\citation{nlmeans}
\citation{irani}
\citation{BM3D}
\citation{bayesnlmeans_kervrann}
\citation{nlbayes}
\citation{WNNM}
\citation{LSSC}
\citation{SAIST}
\citation{NCSR}
\citation{PLR}
\citation{nlmeans_kervrann}
\citation{tupin}
\citation{OWF}
\citation{nlmeans}
\citation{nlmeans_kervrann}
\citation{localA}
\citation{OWF}
\citation{OWF}
\citation{DCT}
\citation{wavelet}
\citation{wavelet_sure}
\citation{matching_pursuit3}
\citation{matching_pursuit2}
\citation{matching_pursuit}
\citation{TV}
\citation{TV}
\citation{DCT}
\citation{fast_DCT}
\citation{DCT}
\citation{wavelet}
\citation{wavelet_sure}
\citation{wavelet_best}
\citation{wavelet_christine}
\citation{wavelet_best}
\newlabel{owf_risk}{{34}{12}}
\newlabel{owf_upper_bound}{{35}{12}}
\@writefile{toc}{\contentsline {subsection}{\numberline {\unhbox \voidb@x \hbox {III-B}}Sparsity methods}{12}\protected@file@percent }
\@writefile{toc}{\contentsline {subsubsection}{\numberline {\unhbox \voidb@x \hbox {III-B}1}Sparsity in a fixed basis}{12}\protected@file@percent }
\newlabel{sparsity_optimization}{{38}{12}}
\@writefile{toc}{\contentsline {paragraph}{\numberline {\unhbox \voidb@x \hbox {III-B}1a}TV denoising}{12}\protected@file@percent }
\citation{BM3D}
\citation{DCT}
\citation{wavelet}
\citation{wavelet_sure}
\citation{BM3D}
\citation{nlbayes}
\citation{WNNM}
\citation{LSSC}
\citation{SAIST}
\citation{NCSR}
\citation{PLR}
\citation{DCT}
\citation{wavelet_best2}
\citation{surelet}
\citation{ksvd}
\citation{ksvd}
\citation{matching_pursuit3}
\citation{matching_pursuit2}
\citation{matching_pursuit}
\citation{eckart}
\citation{ksvd}
\@writefile{toc}{\contentsline {paragraph}{\numberline {\unhbox \voidb@x \hbox {III-B}1b}DCT and DWT denoiser}{13}\protected@file@percent }
\@writefile{toc}{\contentsline {paragraph}{\numberline {\unhbox \voidb@x \hbox {III-B}1c}BM3D}{13}\protected@file@percent }
\@writefile{toc}{\contentsline {subsubsection}{\numberline {\unhbox \voidb@x \hbox {III-B}2}Sparsity on a learned dictionary}{13}\protected@file@percent }
\@writefile{lof}{\contentsline {figure}{\numberline {7}{\ignorespaces Grouping technique for image denoising}}{13}\protected@file@percent }
\newlabel{bm0_2}{{7}{13}}
\@writefile{toc}{\contentsline {paragraph}{\numberline {\unhbox \voidb@x \hbox {III-B}2a}KSVD}{13}\protected@file@percent }
\newlabel{ksvd_optimization}{{40}{13}}
\newlabel{Y-DTheta}{{41}{13}}
\citation{ksvd}
\citation{ksvd2}
\citation{ksvd}
\citation{ksvd2}
\citation{ksvd}
\citation{ksvd}
\citation{BM3D}
\citation{ksvd}
\citation{LSSC}
\citation{SAIST}
\citation{WNNM}
\citation{PLR}
\citation{eckart}
\citation{rank_unconstrained}
\citation{PLR}
\citation{PLR}
\citation{LSSC}
\citation{SAIST}
\citation{NNM}
\citation{WNNM}
\citation{iterative_regularization}
\citation{hyperprior}
\citation{EPLL}
\citation{nlbayes}
\citation{EPLL_unsupervised}
\citation{PLE}
\citation{noise_clinic}
\citation{EPLL}
\citation{nlbayes}
\citation{EPLL}
\citation{EPLL_IPOL}
\citation{EPLL}
\@writefile{lof}{\contentsline {figure}{\numberline {8}{\ignorespaces Data-driven dictionary by KSVD vs overcomplete DCT/Haar dictionaries}}{14}\protected@file@percent }
\newlabel{figure_ksvd}{{8}{14}}
\@writefile{toc}{\contentsline {paragraph}{\numberline {\unhbox \voidb@x \hbox {III-B}2b}Simultaneous sparse coding (SSC) from a low-rank view point}{14}\protected@file@percent }
\newlabel{nnksvd_optimization}{{43}{14}}
\newlabel{nnksvd_optimization_rank}{{44}{14}}
\newlabel{nnksvd_optimization_rank2}{{45}{14}}
\newlabel{nnm_problem}{{46}{14}}
\@writefile{toc}{\contentsline {subsection}{\numberline {\unhbox \voidb@x \hbox {III-C}}Bayesian methods coupled with a Gaussian model}{14}\protected@file@percent }
\@writefile{toc}{\contentsline {paragraph}{\numberline {\unhbox \voidb@x \hbox {III-C}0a}EPLL}{14}\protected@file@percent }
\citation{GemanYang02}
\citation{BoydADMM11}
\citation{EPLL}
\citation{EPLL}
\citation{berkeley}
\citation{EPLL_unsupervised}
\citation{EPLL}
\citation{EPLL_unsupervised}
\citation{deledalle2018image}
\citation{BM3D}
\citation{EPLL}
\citation{FoE}
\citation{PoE}
\citation{nlbayes}
\citation{irani}
\citation{nlbayes}
\citation{nlbayes}
\citation{BM3D}
\citation{noise_clinic}
\citation{S2S}
\citation{DIP}
\citation{N2S}
\citation{DIP}
\citation{S2S}
\citation{DIP}
\citation{DIP}
\citation{DIP}
\citation{DIP}
\citation{TV}
\citation{DIP_TV}
\citation{DIP_RED}
\citation{DIP}
\citation{BM3D}
\citation{RED}
\citation{PnP}
\citation{DIP}
\citation{dip_rita}
\citation{rethinking}
\citation{dip_bayes}
\citation{subdip}
\newlabel{epll_equation}{{49}{15}}
\@writefile{toc}{\contentsline {paragraph}{\numberline {\unhbox \voidb@x \hbox {III-C}0b}NL-Bayes:}{15}\protected@file@percent }
\newlabel{nlbayes_key_equation}{{50}{15}}
\newlabel{nl_bayes_mu_sigma}{{51}{15}}
\@writefile{toc}{\contentsline {subsection}{\numberline {\unhbox \voidb@x \hbox {III-D}}Deep learning-based methods}{15}\protected@file@percent }
\@writefile{toc}{\contentsline {paragraph}{\numberline {\unhbox \voidb@x \hbox {III-D}0a}Deep Image Prior}{15}\protected@file@percent }
\newlabel{dip_equation}{{52}{15}}
\citation{S2S}
\citation{dropout}
\citation{S2S}
\citation{N2S}
\citation{S2S}
\citation{BM3D}
\citation{nlbayes}
\citation{nlridge}
\citation{WNNM}
\citation{SAIST}
\citation{NCSR}
\citation{PEWA}
\citation{OWF}
\citation{equivariant1}
\citation{equivariant_graph2}
\citation{equivariant_graph3}
\citation{equivariant_graph4}
\citation{equivariant_image}
\citation{equivariant_image2}
\citation{equivariant_image3}
\citation{equivariant_image4}
\citation{equivariant_pointcloud1}
\citation{equivariant_pointcloud2}
\citation{equivariant_pointcloud3}
\citation{equivariant_translation1}
\citation{equivariant_translation2}
\citation{homogeneous_functions}
\citation{nlridge}
\citation{lichi}
\@writefile{toc}{\contentsline {paragraph}{\numberline {\unhbox \voidb@x \hbox {III-D}0b}Self2Self}{16}\protected@file@percent }
\newlabel{slef2self}{{53}{16}}
\@writefile{toc}{\contentsline {section}{\numberline {IV}Normalization-equivariance property of denoising methods}{16}\protected@file@percent }
\@writefile{toc}{\contentsline {subsection}{\numberline {\unhbox \voidb@x \hbox {IV-A}}Normalization-equivariance of conventional denoisers}{16}\protected@file@percent }
\newlabel{normalization-equivariance}{{1}{16}}
\@writefile{toc}{\contentsline {subsection}{\numberline {\unhbox \voidb@x \hbox {IV-B}}The case of neural networks}{16}\protected@file@percent }
\citation{normalization_morel}
\citation{SHneurips23}
\citation{TV}
\citation{nlmeans}
\citation{nlridge}
\citation{lichi}
\citation{DCT}
\citation{BM3D}
\citation{WNNM}
\citation{dncnn}
\citation{drunet}
\citation{nlrn}
\citation{swinir}
\citation{DCT}
\citation{BM3D}
\citation{drunet}
\citation{homogeneous_functions}
\citation{restormer}
\citation{n3net}
\citation{nlrn}
\citation{swinir}
\citation{transformer_eccv}
\citation{scunet}
\citation{SHneurips23}
\citation{SHneurips23}
\citation{SHneurips23}
\citation{SHneurips23}
\citation{SHneurips23}
\citation{BM3D}
\citation{nlbayes}
\citation{WNNM}
\citation{lichi}
\citation{scunet}
\citation{WNNM}
\citation{lichi}
\citation{convnext}
\citation{convmixer}
\citation{dead}
\citation{dead2}
\citation{dead3}
\citation{SHneurips23}
\citation{SHneurips23}
\bibstyle{abbrv}
\bibdata{biblio_retouchee}
\bibcite{fully_synthetic_training}{1}
\bibcite{hyperprior}{2}
\bibcite{dset_div2k}{3}
\bibcite{ksvd2}{4}
\newlabel{case_of_nn}{{1}{17}}
\@writefile{toc}{\contentsline {subsection}{\numberline {\unhbox \voidb@x \hbox {IV-C}}Categorizing image denoisers}{17}\protected@file@percent }
\@writefile{lot}{\contentsline {table}{\numberline {I}{\ignorespaces Equivariance properties of several image denoisers}}{17}\protected@file@percent }
\newlabel{properties_summary}{{I}{17}}
\@writefile{lof}{\contentsline {figure}{\numberline {9}{\ignorespaces Impact of normalization for deep-learning-based denoising (DnCNN). All four intervals are subsets of the interval $[0,1]$. Source: \cite  {SHneurips23}.}}{17}\protected@file@percent }
\newlabel{FigEquivData}{{9}{17}}
\@writefile{toc}{\contentsline {section}{\numberline {V}Conclusion}{17}\protected@file@percent }
\@writefile{toc}{\contentsline {section}{References}{17}\protected@file@percent }
\bibcite{ridnet}{5}
\bibcite{N2S}{6}
\bibcite{equivariant_graph4}{7}
\bibcite{surelet}{8}
\bibcite{BoulangerTMI2010}{9}
\bibcite{BoydADMM11}{10}
\bibcite{unprocessing}{11}
\bibcite{nlmeans2}{12}
\bibcite{nlmeans}{13}
\bibcite{mlp}{14}
\bibcite{equivariant_pointcloud3}{15}
\bibcite{NNM}{16}
\bibcite{PNGAN}{17}
\bibcite{noise2noise_improved}{18}
\bibcite{canny}{19}
\bibcite{wavelet_christine}{20}
\bibcite{dead}{21}
\bibcite{transformer_eccv}{22}
\bibcite{matching_pursuit3}{23}
\bibcite{fast_DCT}{24}
\bibcite{tnrd}{25}
\bibcite{dip_bayes}{26}
\bibcite{wavelet}{27}
\bibcite{equivariant1}{28}
\bibcite{mlp_universal3}{29}
\bibcite{BM3D}{30}
\bibcite{tupin}{31}
\bibcite{deledalle2018image}{32}
\bibcite{SAIST}{33}
\bibcite{NCSR}{34}
\bibcite{nlmeans_parameters}{35}
\bibcite{eckart}{36}
\bibcite{tweedie}{37}
\bibcite{ksvd}{38}
\bibcite{ReviewElad2023}{39}
\bibcite{dip_rita}{40}
\bibcite{jpeg_deblocking}{41}
\bibcite{poisson_estimation}{42}
\bibcite{equivariant_pointcloud2}{43}
\bibcite{equivariant_translation1}{44}
\bibcite{mlp_universal2}{45}
\bibcite{GemanYang02}{46}
\bibcite{matching_pursuit2}{47}
\bibcite{WNNM}{48}
\bibcite{equivariant_image4}{49}
\bibcite{photon_noise}{50}
\bibcite{resnet}{51}
\bibcite{nlridge}{52}
\bibcite{lichi}{53}
\@writefile{lof}{\contentsline {figure}{\numberline {10}{\ignorespaces Proposed methodology for designing normalization-equivariant neural networks}}{18}\protected@file@percent }
\newlabel{sortpooling_intro}{{10}{18}}
\bibcite{SHneurips23}{54}
\bibcite{PoE}{55}
\bibcite{rank_unconstrained}{56}
\bibcite{mlp_universal1}{57}
\bibcite{PLR}{58}
\bibcite{EPLL_IPOL}{59}
\bibcite{batchnorm}{60}
\bibcite{OWF}{61}
\bibcite{rethinking}{62}
\bibcite{equivariant_graph2}{63}
\bibcite{PEWA}{64}
\bibcite{nlmeans_kervrann}{65}
\bibcite{localA}{66}
\bibcite{bayesnlmeans_kervrann}{67}
\bibcite{noise2score}{68}
\bibcite{adam}{69}
\bibcite{N2V}{70}
\bibcite{pN2V}{71}
\bibcite{laine}{72}
\bibcite{nlbayes}{73}
\bibcite{noise_clinic}{74}
\bibcite{equivariant_translation2}{75}
\bibcite{N2K}{76}
\bibcite{noise2noise}{77}
\bibcite{DIP}{78}
\bibcite{dead2}{79}
\bibcite{dead3}{80}
\bibcite{swinir}{81}
\bibcite{dset_flickr2k}{82}
\bibcite{score_approx}{83}
\bibcite{nlrn}{84}
\bibcite{EPLL_unsupervised}{85}
\bibcite{DIP_TV}{86}
\bibcite{mwcnn}{87}
\bibcite{swin}{88}
\bibcite{convnext}{89}
\bibcite{wavelet_best2}{90}
\bibcite{wavelet_sure}{91}
\bibcite{dset_waterloo}{92}
\bibcite{LSSC}{93}
\bibcite{matching_pursuit}{94}
\bibcite{nlmeans3}{95}
\bibcite{red30}{96}
\bibcite{equivariant_image}{97}
\bibcite{berkeley}{98}
\bibcite{DIP_RED}{99}
\bibcite{averaging_filters}{100}
\bibcite{homogeneous_functions}{101}
\bibcite{noisier2noise}{102}
\bibcite{MakitaloTIP2011}{103}
\bibcite{iterative_regularization}{104}
\bibcite{R2R}{105}
\bibcite{pytorch}{106}
\bibcite{n3net}{107}
\bibcite{DND}{108}
\bibcite{wavelet_best}{109}
\bibcite{convallaria}{110}
\bibcite{S2S}{111}
\bibcite{monte_carlo_sure}{112}
\bibcite{sgd}{113}
\bibcite{RED}{114}
\bibcite{unet}{115}
\bibcite{mlp_inventor}{116}
\bibcite{FoE}{117}
\bibcite{TV}{118}
\bibcite{dset_labelme}{119}
\bibcite{subdip}{120}
\bibcite{these}{121}
\bibcite{yaroslavsky}{122}
\bibcite{equivariant_graph3}{123}
\bibcite{pixelshuffle}{124}
\bibcite{sure_loss}{125}
\bibcite{dropout}{126}
\bibcite{Starck98}{127}
\bibcite{Anscombe}{128}
\bibcite{SURE}{129}
\bibcite{equivariant_pointcloud1}{130}
\bibcite{bilateral}{131}
\bibcite{convmixer}{132}
\bibcite{attention}{133}
\bibcite{equivariant_image3}{134}
\bibcite{PnP}{135}
\bibcite{normalization_morel}{136}
\bibcite{CARE}{137}
\bibcite{equivariant_image2}{138}
\bibcite{dilated}{139}
\bibcite{DCT}{140}
\bibcite{PLE}{141}
\bibcite{restormer}{142}
\bibcite{cycleisp}{143}
\bibcite{scunet}{144}
\bibcite{drunet}{145}
\bibcite{dncnn}{146}
\bibcite{ircnn}{147}
\bibcite{ffdnet}{148}
\bibcite{rnan}{149}
\bibcite{irani}{150}
\bibcite{EPLL}{151}


==> biblio2.tex <==
\begin{thebibliography}{100}

\bibitem{fully_synthetic_training}
R.~Achddou, Y.~Gousseau, and S.~Ladjal.
\newblock Fully synthetic training for image restoration tasks.
\newblock {\em Comp. Vis. Image Underst.}, 233:103723, 2023.

\bibitem{hyperprior}
C.~Aguerrebere, A.~Almansa, Y.~Gousseau, J.~Delon, and P.~Mus{\'e}.
\newblock A hyperprior {B}ayesian approach for solving image inverse problems.
\newblock {\em HAL preprint}, 2014.

\bibitem{dset_div2k}
E.~Agustsson and R.~Timofte.
\newblock {NTIRE 2017 Challenge} on single image super-resolution: Dataset and
  study.
\newblock In {\em Proc. Conf. Comput. Vis. Pattern Recognit.
  Workshops (CVPRW)}, pp. 1122--1131, 2017.

\bibitem{ksvd2}
M.~Aharon, M.~Elad, and A.~Bruckstein.
\newblock {K-SVD}: An algorithm for designing overcomplete dictionaries for
  sparse representation.
\newblock {\em IEEE Trans. Signal Process.}, 54(11):4311--4322,
  2006.

\bibitem{ridnet}
S.~Anwar and N.~Barnes.
\newblock Real image denoising with feature attention.
\newblock In {\em Proc. Int. Conf. Comput. Vis. (ICCV)}, pp. 3155-3164, 2019.

\bibitem{N2S}
J.~Batson and L.~Royer.
\newblock {N}oise2{S}elf: Blind denoising by self-supervision.
\newblock In {\em Proc. Int. Conf. Mach. Learn. (ICML)},
  vol.~97, pp. 524--533, 2019.

\bibitem{equivariant_graph4}
S.~Batzner, A.~Musaelian, L.~Sun, M.~Geiger, J.~P. Mailoa, M.~Kornbluth,
  N.~Molinari, T.~E. Smidt, and B.~Kozinsky.
\newblock E(3)-equivariant graph neural networks for data-efficient and
  accurate interatomic potentials.
\newblock {\em Nature Comm.}, 13(1):2453, 2022.

\bibitem{surelet}
T.~Blu and F.~Luisier.
\newblock {The SURE-LET approach to image denoising}.
\newblock {\em IEEE Trans. Image Process.}, 16(11):2778--2786, 2007.

\bibitem{BoulangerTMI2010}
J.~Boulanger, C.~Kervrann, P.~Bouthemy, P.~Elbau, J.-B. Sibarita, and
  J.~Salamero.
\newblock Patch-based non-local functional for denoising fluorescence
  microscopy image sequences.
\newblock {\em IEEE Trans.  Med. Imaging}, 29(2):442--454, 2010.

\bibitem{BoydADMM11}
S.~Boyd, N.~Parikh, E.~Chu, B.~Peleato, and J.~Eckstein.
\newblock {\em Distributed Optimization and Statistical Learning via the
  Alternating Direction Method of Multipliers}.
\newblock Now Publishers, 2011.

\bibitem{unprocessing}
T.~Brooks, B.~Mildenhall, T.~Xue, J.~Chen, D.~Sharlet, and J.~T. Barron.
\newblock Unprocessing images for learned raw denoising.
\newblock In {\em Proc. Conf. Comput. Vis. Pattern Recognit. (CVPR)}, pp. 11028--11037, 2019.

\bibitem{nlmeans2}
A.~Buades, B.~Coll, and J.-M. Morel.
\newblock A non-local algorithm for image denoising.
\newblock In {\em Proc. Conf. Comput. Vis. Pattern Recognit. (CVPR)}, vol.~2, pp. 60--65, 2005.

\bibitem{nlmeans}
A.~Buades, B.~Coll, and J.-M. Morel.
\newblock A review of image denoising algorithms, with a new one.
\newblock {\em SIAM J. Multisc. Modeling Simul.}, 4(2):490--530, 2005.

\bibitem{mlp}
H.~C. Burger, C.~J. Schuler, and S.~Harmeling.
\newblock Image denoising: Can plain neural networks compete with {BM3D}?
\newblock In {\em Proc. Conf. Comput. Vis. Pattern Recognit. (CVPR)}, pp. 2392--2399, 2012.

\bibitem{equivariant_pointcloud3}
G.~Bökman, F.~Kahla, and A.~Flinth.
\newblock {ZZ-Net}: A universal rotation equivariant architecture for {2D}
  point clouds.
\newblock In {\em Proc. Conf. Comput. Vis. Pattern Recognit. (CVPR)}, pp. 10966--10975, 2022.

\bibitem{NNM}
J.-F. Cai, E.~J. Cand\`{e}s, and Z.~Shen.
\newblock A singular value thresholding algorithm for matrix completion.
\newblock {\em SIAM J. Optim.}, 20(4):1956--1982, 2010.

\bibitem{PNGAN}
Y.~Cai, X.~Hu, H.~Wang, Y.~Zhang, H.~Pfister, and D.~Wei.
\newblock Learning to generate realistic noisy images via pixel-level
  noise-aware adversarial training.
\newblock In {\em Proc. Int. Conf. Neural Inf. Process. Syst. (NeurIPS)},
  vol.~34, pp. 3259--3270, 2021.

\bibitem{noise2noise_improved}
A.~F. Calvarons.
\newblock Improved {Noise2Noise} denoising with limited data.
\newblock In {\em Proc. Conf. Comput. Vis. Pattern Recognit. Workshops (CVPRW)}, pp. 796--805, 2021.

\bibitem{canny}
J.~Canny.
\newblock A computational approach to edge detection.
\newblock {\em IEEE Trans. Pattern Anal. Mach. Intell.},
  8(6):679--698, 1986.

\bibitem{wavelet_christine}
V.~Chappelier and C.~Guillemot.
\newblock Oriented wavelet transform for image compression and denoising.
\newblock {\em IEEE Trans. Image Process.}, 15(10):2892--2903, 2006.

\bibitem{dead}
P.~Chatterjee and P.~Milanfar.
\newblock Is denoising dead?
\newblock {\em IEEE Trans. Image Process.}, 19(4):895--911, 2010.

\bibitem{transformer_eccv}
L.~Chen, X.~Chu, X.~Zhang, and J.~Sun.
\newblock Simple baselines for image restoration.
\newblock In {\em Proc. Eur. Conf. Comput. Vis. (ECCV)}, pp. 17--33,
  2022.

\bibitem{matching_pursuit3}
S.~S. Chen, D.~L. Donoho, and M.~A. Saunders.
\newblock Atomic decomposition by basis pursuit.
\newblock {\em SIAM J. Scient. Comput.}, 20(1):33--61, 1998.

\bibitem{fast_DCT}
W.-H. Chen, C.~Smith, and S.~Fralick.
\newblock A fast computational algorithm for the {D}iscrete {C}osine
  {T}ransform.
\newblock {\em IEEE Trans. Comm.}, 25(9):1004--1009, 1977.

\bibitem{tnrd}
Y.~Chen and T.~Pock.
\newblock Trainable nonlinear reaction diffusion: A flexible framework for fast
  and effective image restoration.
\newblock {\em IEEE Trans. Pattern Anal. Mach. Intell.},
  39(6):1256--1272, 2017.

\bibitem{dip_bayes}
Z.~Cheng, M.~Gadelha, S.~Maji, and D.~Sheldon.
\newblock A {B}ayesian perspective on the {D}eep {I}mage {P}rior.
\newblock In {\em Proc. Conf. Comput. Vis. Pattern Recognit. (CVPR)}, June 2019.

\bibitem{wavelet}
H.~A. Chipman, E.~D. Kolaczyk, and R.~E. McCulloch.
\newblock {Adaptive Bayesian wavelet shrinkage}.
\newblock {\em J. Am. Statist. Assoc.},
  92(440):1413--1421, 1997.

\bibitem{equivariant1}
T.~Cohen and M.~Welling.
\newblock Group equivariant convolutional networks.
\newblock In {\em Proc. Int. Conf. Mach. Learn. (ICML)},
  vol.~48, pp. 2990--2999, 2016.

\bibitem{mlp_universal3}
G.~Cybenko.
\newblock Approximation by superpositions of a sigmoidal function.
\newblock {\em Math. Control, Signals, Syst.}, 2(4):303--314,
  1989.

\bibitem{BM3D}
K.~Dabov, A.~Foi, V.~Katkovnik, and K.~Egiazarian.
\newblock {Image denoising by sparse 3-D transform-domain collaborative
  filtering}.
\newblock {\em IEEE Trans. Image Process.}, 16(8):2080--2095, 2007.

\bibitem{tupin}
C.-A. Deledalle, L.~Denis, and F.~Tupin.
\newblock Iterative weighted maximum likelihood denoising with probabilistic
  patch-based weights.
\newblock {\em IEEE Trans. Image Process.}, 18(12):2661--2672, 2009.

\bibitem{deledalle2018image}
C.-A. Deledalle, S.~Parameswaran, and T.~Q. Nguyen.
\newblock Image denoising with generalized {G}aussian mixture model patch
  priors.
\newblock {\em SIAM J. Imaging Sci.}, 11(4):2568--2609, 2018.

\bibitem{SAIST}
W.~Dong, G.~Shi, and X.~Li.
\newblock Nonlocal image restoration with bilateral variance estimation: A
  low-rank approach.
\newblock {\em IEEE Trans. Image Process.}, 22(2):700--711, 2013.

\bibitem{NCSR}
W.~Dong, L.~Zhang, G.~Shi, and X.~Li.
\newblock Nonlocally centralized sparse representation for image restoration.
\newblock {\em IEEE Trans. Image Process.}, 22(4):1620--1630, 2013.

\bibitem{nlmeans_parameters}
V.~Duval, J.-F. Aujol, and Y.~Gousseau.
\newblock A bias-variance approach for the nonlocal means.
\newblock {\em SIAM J. Imaging Sci.}, 4(2):760--788, 2011.

\bibitem{eckart}
C.~Eckart and G.~Young.
\newblock The approximation of one matrix by another of lower rank.
\newblock {\em Psychometrika}, 1(3):211--218, 1936.

\bibitem{tweedie}
B.~Efron.
\newblock Tweedie’s formula and selection bias.
\newblock {\em J. Am. Statist. Assoc.},
  106(496):1602--1614, 2011.

\bibitem{ksvd}
M.~Elad and M.~Aharon.
\newblock Image denoising via sparse and redundant representations over learned
  dictionaries.
\newblock {\em IEEE Trans. Image Process.}, 15(12):3736--3745, 2006.

\bibitem{ReviewElad2023}
M.~Elad, B.~Kawar, and G.~Vaksman.
\newblock Image denoising: the deep learning revolution and beyond -- a survey
  paper.
\newblock {\em SIAM J. Imaging Sci.}, 16(3):1594--1654, 2023.

\bibitem{dip_rita}
R.~Fermanian, M.~Le~Pendu, and C.~Guillemot.
\newblock Regularizing the {D}eep {I}mage {P}rior with a learned denoiser for
  linear inverse problems.
\newblock In {\em Proc. Int. Workshop Multimed. Signal Process. (MMSP)}, pp. 1--6, 2021.
\bibitem{jpeg_deblocking}
A.~Foi, V.~Katkovnik, and K.~Egiazarian.
\newblock Pointwise shape-adaptive dct for high-quality deblocking of
  compressed color images.
\newblock In {\em Proc. Eur. Signal Process. Conf. (EUSIPCO)}, pp. 1--5,
  2006.

\bibitem{poisson_estimation}
A.~Foi, M.~Trimeche, V.~Katkovnik, and K.~Egiazarian.
\newblock Practical {Poissonian-Gaussian} noise modeling and fitting for
  single-image raw-data.
\newblock {\em IEEE Trans. Image Process.}, 17(10):1737--1754, 2008.

\bibitem{equivariant_pointcloud2}
F.~Fuchs, D.~Worrall, V.~Fischer, and M.~Welling.
\newblock {SE(3)-Transformers}: {3D} roto-translation equivariant attention
  networks.
\newblock In {\em Proc. Int. Conf. Neural Inf. Process. Syst. (NeurIPS)},
  vol.~33, pp. 1970--1981, 2020.

\bibitem{equivariant_translation1}
K.~Fukushima.
\newblock Neocognitron: A self-organizing neural network model for a mechanism
  of pattern recognition unaffected by shift in position.
\newblock {\em Biol. Cybern.}, 36(4):193--202, 1980.

\bibitem{mlp_universal2}
K.-I. Funahashi.
\newblock On the approximate realization of continuous mappings by neural
  networks.
\newblock {\em Neural Networks}, 2(3):183--192, 1989.

\bibitem{GemanYang02}
D.~Geman and C.~Yang.
\newblock Nonlinear image recovery with half-quadratic regularization.
\newblock {\em IEEE Trans. Image Process.}, 4(7):932--946, 2002.

\bibitem{matching_pursuit2}
I.~Gorodnitsky and B.~Rao.
\newblock Sparse signal reconstruction from limited data using {FOCUSS}: a
  re-weighted minimum norm algorithm.
\newblock {\em IEEE Trans. Signal Process.}, 45(3):600--616, 1997.

\bibitem{WNNM}
S.~Gu, L.~Zhang, W.~Zuo, and X.~Feng.
\newblock {Weighted nuclear norm minimization with application to image
  denoising}.
\newblock In {\em Proc. Conf. Comput. Vis. Pattern Recognit. (CVPR)}, pp. 2862--2869, 2014.

\bibitem{equivariant_image4}
D.~K. Gupta, D.~Arya, and E.~Gavves.
\newblock Rotation equivariant siamese networks for tracking.
\newblock In {\em Proc. Conf. Comput. Vis. Pattern Recognit. (CVPR)}, pp. 12357--12366, 2021.

\bibitem{photon_noise}
S.~W. Hasinoff.
\newblock Photon, {Poisson} noise.
\newblock {\em Computer Vision, A Reference Guide}, 4(16):1, 2014.

\bibitem{resnet}
K.~He, X.~Zhang, S.~Ren, and J.~Sun.
\newblock Deep residual learning for image recognition.
\newblock In {\em Proc. Conf. Comput. Vis. Pattern Recognit. (CVPR)}, pp. 770--778, 2016.

\bibitem{nlridge}
S.~Herbreteau and C.~Kervrann.
\newblock Towards a unified view of unsupervised non-local methods for image
  denoising: the {NL-Ridge} approach.
\newblock In {\em Proc. Int. Conf. Image Process. (ICIP)},
  pp. 3376--3380, 2022.

\bibitem{lichi}
S.~Herbreteau and C.~Kervrann.
\newblock Unsupervised linear and iterative combinations of patches for image
  denoising.
\newblock {\em arXiv preprint arXiv:2212.00422}, 2022.

\bibitem{SHneurips23}
S.~Herbreteau, E.~Moebel, and C.~Kervrann.
\newblock Normalization-equivariant neural networks with application to image
  denoising.
\newblock In {\em Proc. Int. Conf. Neural Inf. Process. Syst. (NeurIPS)}, New-Orleans, USA, 2023.

\bibitem{PoE}
G.~Hinton.
\newblock Products of experts.
\newblock In {\em International Conference on Artificial Neural Networks
  (ICANN)}, vol.~1, pp. 1--6, 1999.

\bibitem{rank_unconstrained}
J.-B. Hiriart-Urruty and H.~Y. Le.
\newblock From eckart and young approximation to {M}oreau envelopes and vice
  versa.
\newblock {\em RAIRO-Operations Research},
  47(3):299--310, 2013.

\bibitem{mlp_universal1}
K.~Hornik, M.~Stinchcombe, and H.~White.
\newblock Multilayer feedforward networks are universal approximators.
\newblock {\em Neural Networks}, 2(5):359--366, 1989.

\bibitem{PLR}
H.~Hu, J.~Froment, and Q.~Liu.
\newblock A note on patch-based low-rank minimization for fast image denoising.
\newblock {\em J. Visual Comm. Image Repres.},
  50:100--110, 2018.

\bibitem{EPLL_IPOL}
S.~Hurault, T.~Ehret, and P.~Arias.
\newblock {EPLL}: an image denoising method using a {G}aussian mixture model
  learned on a large set of patches.
\newblock {\em {Image Process. On Line}}, 8:465--489, 2018.

\bibitem{batchnorm}
S.~Ioffe and C.~Szegedy.
\newblock Batch normalization: Accelerating deep network training by reducing
  internal covariate shift.
\newblock In {\em Proc. Int. Conf. Mach. Learn. (ICML)},
  vol.~37, pp. 448--456, 2015.

\bibitem{OWF}
Q.~Jin, I.~Grama, C.~Kervrann, and Q.~Liu.
\newblock Nonlocal means and optimal weights for noise removal.
\newblock {\em SIAM J. Imaging Sci.}, 10(4):1878--1920, 2017.

\bibitem{rethinking}
Y.~Jo, S.~Y. Chun, and J.~Choi.
\newblock Rethinking {D}eep {I}mage {P}rior for denoising.
\newblock In {\em Proc. Int. Conf. Comput. Vis. (ICCV)}, pp.
  5087--5096, 2021.

\bibitem{equivariant_graph2}
N.~Keriven and G.~Peyr\'{e}.
\newblock Universal invariant and equivariant graph neural networks.
\newblock In {\em Proc. Int. Conf. Neural Inf. Process. Syst. (NeurIPS)},
  vol.~32, 2019.

\bibitem{PEWA}
C.~Kervrann.
\newblock {PEWA}: Patch-based exponentially weighted aggregation for image
  denoising.
\newblock In {\em Proc. Int. Conf. Adv. Neural Inf. Process. Syst. (NIPS)},
  vol.~27, 2014.

\bibitem{nlmeans_kervrann}
C.~Kervrann and J.~Boulanger.
\newblock Optimal spatial adaptation for patch-based image denoising.
\newblock {\em IEEE Trans. Image Process.}, 15(10):2866--2878, 2006.

\bibitem{localA}
C.~Kervrann and J.~Boulanger.
\newblock Local adaptivity to variable smoothness for exemplar-based image
  regularization and representation.
\newblock {\em Int. J. Comput. Vis.}, 79(1):45--69, 2008.

\bibitem{bayesnlmeans_kervrann}
C.~Kervrann, J.~Boulanger, and P.~Coupé.
\newblock Bayesian non-local means filter, image redundancy and adaptive
  dictionaries for noise removal.
\newblock In {\em Proc. Int. Conf. Scale Space Variational Methods Comput. Vis.},
  pp. 520--532, 2007.

\bibitem{noise2score}
K.~Kim and J.~C. Ye.
\newblock {Noise2Score}: {Tweedie’s} approach to self-supervised image
  denoising without clean images.
\newblock In {\em Proc. Int. Conf. Neural Inf. Process. Syst. (NeurIPS)},
  vol.~34, pp. 864--874, 2021.

\bibitem{adam}
D.~Kingma and J.~Ba.
\newblock Adam: A method for stochastic optimization.
\newblock In {\em Proc. Int. Conf. Learn. Representations (ICLR)},
  2015.

\bibitem{N2V}
A.~Krull, T.-O. Buchholz, and F.~Jug.
\newblock {Noise2Void - Learning denoising from single noisy images}.
\newblock In {\em Proc. Conf. Comput. Vis. Pattern Recognit. (CVPR)}, pp. 2124--2132, 2019.

\bibitem{pN2V}
A.~Krull, T.~Vicar, M.~Prakash, M.~Lalit, and F.~Jug.
\newblock Probabilistic {Noise2Void}: Unsupervised content-aware denoising.
\newblock {\em Frontiers Comput. Sci.}, 2:5, 2020.

\bibitem{laine}
S.~Laine, T.~Karras, J.~Lehtinen, and T.~Aila.
\newblock High-quality self-supervised deep image denoising.
\newblock In {\em Proc. Int. Conf. Neural Inf. Process. Syst. (NeurIPS)},
  vol.~32, 2019.

\bibitem{nlbayes}
M.~Lebrun, A.~Buades, and J.~M. Morel.
\newblock {A nonlocal Bayesian image denoising algorithm}.
\newblock {\em SIAM J. Imaging Sci.}, 6(3):1665--1688, 2013.

\bibitem{noise_clinic}
M.~Lebrun, M.~Colom, and J.-M. Morel.
\newblock {The Noise Clinic}: a blind image denoising algorithm.
\newblock {\em {Image Process. On Line}}, 5:1--54, 2015.

\bibitem{equivariant_translation2}
Y.~LeCun, B.~Boser, J.~S. Denker, D.~Henderson, R.~E. Howard, W.~Hubbard, and
  L.~D. Jackel.
\newblock Backpropagation applied to handwritten zip code recognition.
\newblock {\em Neural Computation}, 1(4):541--551, 1989.

\bibitem{N2K}
K.~Lee and W.-K. Jeong.
\newblock {Noise2Kernel}: Adaptive self-supervised blind denoising using a
  dilated convolutional kernel architecture.
\newblock {\em Sensors}, 22(11):4255, 2022.

\bibitem{noise2noise}
J.~Lehtinen, J.~Munkberg, J.~Hasselgren, S.~Laine, T.~Karras, M.~Aittala, and
  T.~Aila.
\newblock {N}oise2{N}oise: Learning image restoration without clean data.
\newblock In {\em Proc. Int. Conf. Mach. Learn. (ICML)},
  vol.~80, pp. 2965--2974, 2018.

\bibitem{DIP}
V.~Lempitsky, A.~Vedaldi, and D.~Ulyanov.
\newblock Deep image prior.
\newblock In {\em Proc. Conf. Comput. Vis. Pattern Recognit. (CVPR)}, pp. 9446--9454, 2018.

\bibitem{dead2}
A.~Levin and B.~Nadler.
\newblock Natural image denoising: Optimality and inherent bounds.
\newblock In {\em Proc. Conf. Comput. Vis. Pattern Recognit. (CVPR)}, pp. 2833--2840, 2011.

\bibitem{dead3}
A.~Levin, B.~Nadler, F.~Durand, and W.~T. Freeman.
\newblock Patch complexity, finite pixel correlations and optimal denoising.
\newblock In {\em Proc. Eur. Conf. Comput. Vis. (ECCV)}, pp. 73--86,
  2012.

\bibitem{swinir}
J.~Liang, J.~Cao, G.~Sun, K.~Zhang, L.~Van~Gool, and R.~Timofte.
\newblock {SwinIR}: Image restoration using {Swin Transformer}.
\newblock In {\em Proc. Int. Conf. Comput. Vis. Workshops (ICCVW)}, pp. 1833--1844, 2021.

\bibitem{dset_flickr2k}
B.~Lim, S.~Son, H.~Kim, S.~Nah, and K.~M. Lee.
\newblock Enhanced deep residual networks for single image super-resolution.
\newblock In {\em Proc. Conf. Comput. Vis. Pattern Recognit. Workshops (CVPRW)}, pp. 1132--1140, 2017.

\bibitem{score_approx}
J.~H. Lim, A.~Courville, C.~Pal, and C.-W. Huang.
\newblock {AR}-{DAE}: Towards unbiased neural entropy gradient estimation.
\newblock In {\em Int. Conf. Mach. Learn. (ICML)}, vol.
  119, pp. 6061--6071, 2020.

\bibitem{nlrn}
D.~Liu, B.~Wen, Y.~Fan, C.~C. Loy, and T.~S. Huang.
\newblock Non-local recurrent network for image restoration.
\newblock In {\em roc. Int. Conf. Neural Inf. Process. Syst. (NeurIPS)},
  vol.~31, 2018.

\bibitem{EPLL_unsupervised}
H.~Liu, X.~Liu, J.~Lu, and S.~Tan.
\newblock Self-supervised image prior learning with {GMM} from a single noisy
  image.
\newblock In {\em Proc. Int. Conf. Comput. Vis. (ICCV)}, pp.
  2825--2834, 2021.

\bibitem{DIP_TV}
J.~Liu, Y.~Sun, X.~Xu, and U.~S. Kamilov.
\newblock Image restoration using total variation regularized deep image prior.
\newblock In {\em Proc. Int. Conf. Ac. Speech Signal Process. (ICASSP)}, pp. 7715--7719, 2019.

\bibitem{mwcnn}
P.~Liu, H.~Zhang, K.~Zhang, L.~Lin, and W.~Zuo.
\newblock {Multi-level wavelet-CNN for image restoration}.
\newblock In {\em Proc. Conf. Comput. Vis. Pattern Recognit. Workshops (CVPRW)}, pp. 773--782, 2018.

\bibitem{swin}
Z.~Liu, Y.~Lin, Y.~Cao, H.~Hu, Y.~Wei, Z.~Zhang, S.~Lin, and B.~Guo.
\newblock {Swin Transformer}: Hierarchical vision {Transformer} using shifted
  windows.
\newblock In {\em Proc. Int. Conf. Comput. Vis. (ICCV)}, pp.
  9992--10002, 2021.

\bibitem{convnext}
Z.~Liu, H.~Mao, C.-Y. Wu, C.~Feichtenhofer, T.~Darrell, and S.~Xie.
\newblock A {ConvNet} for the 2020s.
\newblock In {\em Proc. Conf. Comput. Vis. Pattern Recognit. (CVPR)}, pp. 11966--11976, 2022.

\bibitem{wavelet_best2}
F.~Luisier, T.~Blu, B.~Forster, and M.~Unser.
\newblock {Which wavelet bases are the best for image denoising?}
\newblock In {\em Wavelets XI}, vol. 5914, page 59140E, 2005.

\bibitem{wavelet_sure}
F.~Luisier, T.~Blu, and M.~Unser.
\newblock A new {SURE} approach to image denoising: interscale orthonormal
  wavelet thresholding.
\newblock {\em IEEE Trans.Image Process.}, 16(3):593--606, 2007.

\bibitem{dset_waterloo}
K.~Ma, Z.~Duanmu, Q.~Wu, Z.~Wang, H.~Yong, H.~Li, and L.~Zhang.
\newblock Waterloo exploration database: New challenges for image quality
  assessment models.
\newblock {\em IEEE Trans. Image Process.}, 26(2):1004--1016, 2017.

\bibitem{LSSC}
J.~Mairal, F.~Bach, J.~Ponce, G.~Sapiro, and A.~Zisserman.
\newblock Non-local sparse models for image restoration.
\newblock In {\em Proc. Int. Conf. Comput. Vis. (ICCV)}, pp.
  2272--2279, 2009.

\bibitem{matching_pursuit}
S.~Mallat and Z.~Zhang.
\newblock Matching pursuits with time-frequency dictionaries.
\newblock {\em IEEE Trans. ignal Process.}, 41(12):3397--3415,
  1993.

\bibitem{nlmeans3}
J.~V. Manj{\'o}n, J.~Carbonell-Caballero, J.~J. Lull,
  G.~Garc{\'\i}a-Mart{\'\i}, L.~Mart{\'\i}-Bonmat{\'\i}, and M.~Robles.
\newblock {MRI denoising using non-local means}.
\newblock {\em Med. Image Anal.}, 12(4):514--523, 2008.

\bibitem{red30}
X.~Mao, C.~Shen, and Y.-B. Yang.
\newblock Image restoration using very deep convolutional encoder-decoder
  networks with symmetric skip connections.
\newblock In {\em Proc. Int. Conf. Adv. Neural Inf. Process. Syst. (NIPS)},
  vol.~29, 2016.

\bibitem{equivariant_image}
D.~Marcos, M.~Volpi, N.~Komodakis, and D.~Tuia.
\newblock Rotation equivariant vector field networks.
\newblock In {\em Proc. Int. Conf. Comput. Vis. (ICCV)}, pp.
  5058--5067, 2017.

\bibitem{berkeley}
D.~Martin, C.~Fowlkes, D.~Tal, and J.~Malik.
\newblock A database of human segmented natural images and its application to
  evaluating segmentation algorithms and measuring ecological statistics.
\newblock In {\em Proc. Int. Conf. Comput. Vis. (ICCV)},
  vol.~2, pp. 416--423 vol.2, 2001.

\bibitem{DIP_RED}
G.~Mataev, P.~Milanfar, and M.~Elad.
\newblock {DeepRED}: Deep image prior powered by {RED}.
\newblock In {\em Proc. Int. Conf. Comput. Vis. Workshops
  (ICCVW)}, 2019.

\bibitem{averaging_filters}
P.~Milanfar.
\newblock Symmetrizing smoothing filters.
\newblock {\em SIAM J. Imaging Sci.}, 6(1):263--284, 2013.

\bibitem{homogeneous_functions}
S.~Mohan, Z.~Kadkhodaie, E.~P. Simoncelli, and C.~Fernandez-Granda.
\newblock Robust and interpretable blind image denoising via bias-free
  convolutional neural networks.
\newblock In {\em Proc. Int. Conf. Learn. Representations (ICLR)},
  2020.

\bibitem{noisier2noise}
N.~Moran, D.~Schmidt, Y.~Zhong, and P.~Coady.
\newblock {Noisier2Noise}: Learning to denoise from unpaired noisy data.
\newblock In {\em Proc. Conf. Comput. Vis. Pattern Recognit. (CVPR)}, pp. 12061--12069, 2020.

\bibitem{MakitaloTIP2011}
M.~Mäkitalo and A.~Foi.
\newblock A closed-form approximation of the exact unbiased inverse of the
  anscombe variance-stabilizing transformation.
\newblock {\em IEEE Trans. Image Process.}, 20(9):2697--2698, 2011.

\bibitem{iterative_regularization}
S.~Osher, M.~Burger, D.~Goldfarb, J.~Xu, and W.~Yin.
\newblock An iterative regularization method for total variation-based image
  restoration.
\newblock {\em SIAM J. Multisc. Modeling Simul.}, 4(2):460--489, 2005.

\bibitem{R2R}
T.~Pang, H.~Zheng, Y.~Quan, and H.~Ji.
\newblock {Recorrupted-to-Recorrupted}: Unsupervised deep learning for image
  denoising.
\newblock In {\em Proc. Conf. Comput. Vis. Pattern Recognit. (CVPR)}, pp. 2043--2052, 2021.

\bibitem{pytorch}
A.~Paszke, S.~Gross, F.~Massa, A.~Lerer, J.~Bradbury, G.~Chanan, T.~Killeen,
  Z.~Lin, N.~Gimelshein, L.~Antiga, A.~Desmaison, A.~Kopf, E.~Yang, Z.~DeVito,
  M.~Raison, A.~Tejani, S.~Chilamkurthy, B.~Steiner, L.~Fang, J.~Bai, and
  S.~Chintala.
\newblock {PyTorch}: An imperative style, high-performance deep learning
  library.
\newblock In {\em Proc. Int. Conf. Neural Inf. Process. Syst. (NeurIPS)},
  vol.~32, 2019.

\bibitem{n3net}
T.~Pl\"{o}tz and S.~Roth.
\newblock Neural nearest neighbors networks.
\newblock In {\em Proc. Int. Conf. Neural Inf. Process. Syst. (NeurIPS)},
  vol.~31, 2018.

\bibitem{DND}
T.~Plötz and S.~Roth.
\newblock Benchmarking denoising algorithms with real photographs.
\newblock In {\em Proc. Conf. Comput. Vis. Pattern Recognit. (CVPR)}, pp. 2750--2759, 2017.

\bibitem{wavelet_best}
J.~Portilla, V.~Strela, M.~Wainwright, and E.~Simoncelli.
\newblock {Image denoising using scale mixtures of Gaussians in the wavelet
  domain}.
\newblock {\em IEEE Trans. Image Process.}, 12(11):1338--1351, 2003.

\bibitem{convallaria}
M.~Prakash, M.~Lalit, P.~Tomancak, A.~Krul, and F.~Jug.
\newblock Fully unsupervised probabilistic {Noise2Void}.
\newblock In {\em Proc. Int. Symp. Biomed. Imaging (ISBI)}, pp.
  154--158, 2020.

\bibitem{S2S}
Y.~Quan, M.~Chen, T.~Pang, and H.~Ji.
\newblock {Self2Self} with dropout: Learning self-supervised denoising from
  single image.
\newblock In {\em Proc. Conf. Comput. Vis. Pattern Recognit. (CVPR)}, pp. 1887--1895, 2020.

\bibitem{monte_carlo_sure}
S.~Ramani, T.~Blu, and M.~Unser.
\newblock {Monte-Carlo SURE}: A black-box optimization of regularization
  parameters for general denoising algorithms.
\newblock {\em IEEE Trans. Image Process.}, 17(9):1540--1554, 2008.

\bibitem{sgd}
H.~Robbins and S.~Monro.
\newblock A stochastic approximation method.
\newblock {\em The Annals Math. Statist.}, pp. 400--407, 1951.

\bibitem{RED}
Y.~Romano, M.~Elad, and P.~Milanfar.
\newblock {The little engine that could: Regularization by Denoising (RED)}.
\newblock {\em SIAM J. Imaging Sci.}, 10(4):1804--1844, 2017.

\bibitem{unet}
O.~Ronneberger, P.~Fischer, and T.~Brox.
\newblock {U-Net}: Convolutional networks for biomedical image segmentation.
\newblock In {\em Proc.  Int. Conf.  Med. Image Comput. Computer Assisted Intervention
  (MICCAI)}, pp. 234--241, 2015.

\bibitem{mlp_inventor}
F.~Rosenblatt.
\newblock The perceptron: a probabilistic model for information storage and
  organization in the brain.
\newblock {\em Psychol. Rev.}, 65(6):386, 1958.

\bibitem{FoE}
S.~Roth and M.~Black.
\newblock {Fields of Experts}: a framework for learning image priors.
\newblock In {\em CProc. Conf. Comput. Vis. Pattern Recognit. (CVPR)}, vol.~2, pp. 860--867, 2005.

\bibitem{TV}
L.~Rudin, S.~Osher, and E.~Fatemi.
\newblock Nonlinear total variation based noise removal algorithms.
\newblock {\em Physica D: Nonlin. Phenomena}, 60:259--268, 1992.

\bibitem{dset_labelme}
B.~C. Russell, A.~Torralba, K.~P. Murphy, and W.~T. Freeman.
\newblock {LabelMe}: a database and web-based tool for image annotation.
\newblock {\em Int. J. Comput. Vis.}, 77:157--173, 2008.

\bibitem{subdip}
A.~Sagel, A.~Roumy, and C.~Guillemot.
\newblock Sub-dip: Optimization on a subspace with deep image prior
  regularization and application to superresolution.
\newblock In {\em Proc. Int. Conf. Ac. Speech Signal Process. (ICASSP)}, pp. 2513--2517, 2020.

\bibitem{these}
J.~Salmon.
\newblock {\em Agrégation d’estimateurs et méthodes à patch pour le
  débruitage d’images numériques}.
\newblock PhD thesis, University Paris Diderot, 2010.

\bibitem{yaroslavsky}
J.~Salmon, R.~Willett, and E.~Arias-Castro.
\newblock A two-stage denoising filter: The preprocessed {Yaroslavsky} filter.
\newblock In {\em Proc. Int. Workshop Statist. Signal Process. (SSP)}, pp.
  464--467, 2012.

\bibitem{equivariant_graph3}
V.~G. Satorras, E.~Hoogeboom, and M.~Welling.
\newblock E(n) equivariant graph neural networks.
\newblock In {\em Proc. Int. Conf. Mach. Lear. (ICML)}, vol.
  139, pp. 9323--9332, 2021.

\bibitem{pixelshuffle}
W.~Shi, J.~Caballero, F.~Huszár, J.~Totz, A.~P. Aitken, R.~Bishop,
  D.~Rueckert, and Z.~Wang.
\newblock Real-time single image and video super-resolution using an efficient
  sub-pixel convolutional neural network.
\newblock In {\em Proc. Conf. Comput. Vis. Pattern Recognit. (CVPR)}, pp. 1874--1883, 2016.

\bibitem{sure_loss}
S.~Soltanayev and S.~Y. Chun.
\newblock Training deep learning based denoisers without ground truth data.
\newblock In {\em Proc. Int. Conf. Neural Inf. Process. Syst. (NeurIPS)},
  vol.~31, 2018.

\bibitem{dropout}
N.~Srivastava, G.~Hinton, A.~Krizhevsky, I.~Sutskever, and R.~Salakhutdinov.
\newblock Dropout: A simple way to prevent neural networks from overfitting.
\newblock {\em J. Mach. Learn. Research}, 15(56):1929--1958, 2014.

\bibitem{Starck98}
J.-L. Starck and F.~Murtagh.
\newblock Automatic noise estimation from the multiresolution support.
\newblock {\em Pub. Astron. Soc. Pacific},
  110:193 – 199, 1998.

\bibitem{Anscombe}
J.-L. Starck, F.~D. Murtagh, and A.~Bijaoui.
\newblock {\em {Image Processing and Data Analysis: the multiscale approach}}.
\newblock Cambridge University Press, 1998.

\bibitem{SURE}
C.~M. Stein.
\newblock Estimation of the mean of a multivariate normal distribution.
\newblock {\em The Annals of Statist.}, 9(6):1135--1151, 1981.

\bibitem{equivariant_pointcloud1}
N.~Thomas, T.~Smidt, S.~Kearnes, L.~Yang, L.~Li, K.~Kohlhoff, and P.~Riley.
\newblock Tensor field networks: Rotation-and translation-equivariant neural
  networks for {3D} point clouds.
\newblock {\em arXiv preprint arXiv:1802.08219}, 2018.

\bibitem{bilateral}
C.~Tomasi and R.~Manduchi.
\newblock Bilateral filtering for gray and color images.
\newblock In {\em Proc. Int. Conf. Comput. Vis. (ICCV)}, pp.
  839--846, 1998.

\bibitem{convmixer}
A.~Trockman and J.~Z. Kolter.
\newblock Patches are all you need?
\newblock {\em arXiv preprint arXiv:2201.09792}, 2022.

\bibitem{attention}
A.~Vaswani, N.~Shazeer, N.~Parmar, J.~Uszkoreit, L.~Jones, A.~N. Gomez,
  L.~Kaiser, and I.~Polosukhin.
\newblock Attention is all you need.
\newblock In {\em Proc. Int. Conf. Neural Inf. Process. Syst. (NeurIPS)},
  vol.~30, 2017. 

\bibitem{equivariant_image3}
B.~S. Veeling, J.~Linmans, J.~Winkens, T.~Cohen, and M.~Welling.
\newblock Rotation equivariant {CNNs} for digital pathology.
\newblock In {\em Proc.  Int. Conf.  Med. Image Comput. Computer Assist. Interv.(MICCAI)}, pp. 210--218, 2018.

\bibitem{PnP}
S.~V. Venkatakrishnan, C.~A. Bouman, and B.~Wohlberg.
\newblock {Plug-and-Play} priors for model based reconstruction.
\newblock In {\em Global Conf. Signal Inf. Process.},
  pp. 945--948, 2013.

\bibitem{normalization_morel}
Y.-Q. Wang and J.-M. Morel.
\newblock Can a single image denoising neural network handle all levels of
  {G}aussian noise?
\newblock {\em IEEE Signal Process. Letters}, 21(9):1150--1153, 2014.

\bibitem{CARE}
M.~Weigert, U.~Schmidt, T.~Boothe, A.~Müller, A.~Dibrov, A.~Jain, B.~Wilhelm,
  D.~Schmidt, C.~Broaddus, S.~Culley, M.~Rocha-Martins, F.~Segovia-Miranda,
  C.~Norden, R.~Henriques, M.~Zerial, M.~Solimena, J.~Rink, P.~Tomancak,
  L.~Royer, and E.~Myers.
\newblock Content-aware image restoration: pushing the limits of fluorescence
  microscopy.
\newblock {\em Nature Meth.}, 15(12):1090--1097, 2018.

\bibitem{equivariant_image2}
M.~Weiler, F.~A. Hamprecht, and M.~Storath.
\newblock Learning steerable filters for rotation equivariant {CNNs}.
\newblock In {\em Proc. Conf. Comput. Vis. Pattern Recognit. (CVPR)}, pp. 849--858, 2018.

\bibitem{dilated}
F.~Yu and V.~Koltun.
\newblock Multi-scale context aggregation by dilated convolutions.
\newblock {\em arXiv preprint arXiv:1511.07122}, 2015.

\bibitem{DCT}
G.~Yu and G.~Sapiro.
\newblock {DCT} image denoising: a simple and effective image denoising
  algorithm.
\newblock {\em {Image Process. On Line}}, 1:292--296, 2011.

\bibitem{PLE}
G.~Yu, G.~Sapiro, and S.~Mallat.
\newblock Solving inverse problems with piecewise linear estimators: From
  {G}aussian mixture models to structured sparsity.
\newblock {\em IEEE Trans. Image Process.}, 21(5):2481--2499, 2012.

\bibitem{restormer}
S.~W. Zamir, A.~Arora, S.~Khan, M.~Hayat, F.~S. Khan, and M.~Yang.
\newblock Restormer: Efficient transformer for high-resolution image
  restoration.
\newblock In {\em Proc. Conf. Comput. Vis. Pattern Recognit. (CVPR)}, pp. 5718--5729, 2022.

\bibitem{cycleisp}
S.~W. Zamir, A.~Arora, S.~Khan, M.~Hayat, F.~S. Khan, M.-H. Yang, and L.~Shao.
\newblock {CycleISP}: Real image restoration via improved data synthesis.
\newblock In {\em Proc. Conf. Comput. Vis. Pattern Recognit. (CVPR)}, pp. 2693--2702, 2020.

\bibitem{scunet}
K.~Zhang, Y.~Li, J.~Liang, J.~Cao, Y.~Zhang, H.~Tang, D.-P. Fan, R.~Timofte,
  and L.~V. Gool.
\newblock {Practical blind image denoising via Swin-Conv-UNet and data
  synthesis}.
\newblock {\em Mach. Intell. Research}, 2023.

\bibitem{drunet}
K.~Zhang, Y.~Li, W.~Zuo, L.~Zhang, L.~Van~Gool, and R.~Timofte.
\newblock {Plug-and-Play} image restoration with deep denoiser prior.
\newblock {\em IEEE Trans. Pattern Anal. Mach. Intell.},
  44(10):6360--6376, 2022.

\bibitem{dncnn}
K.~Zhang, W.~Zuo, Y.~Chen, D.~Meng, and L.~Zhang.
\newblock Beyond a {G}aussian denoiser: residual learning of deep {CNN} for
  image denoising.
\newblock {\em IEEE Trans. Image Process.}, 26(7):3142--3155, 2017.

\bibitem{ircnn}
K.~Zhang, W.~Zuo, S.~Gu, and L.~Zhang.
\newblock {Learning deep CNN denoiser prior for image restoration}.
\newblock In {\em Proc. Conf. Comput. Vis. Pattern Recognit. (CVPR)}, pp. 2808--2817, 2017.

\bibitem{ffdnet}
K.~Zhang, W.~Zuo, and L.~Zhang.
\newblock {FFDNet}: Toward a fast and flexible solution for {CNN}-based image
  denoising.
\newblock {\em IEEE Trans. Image Process.}, 27(9):4608--4622, 2018.

\bibitem{rnan}
Y.~Zhang, K.~Li, K.~Li, B.~Zhong, and Y.~Fu.
\newblock Residual non-local attention networks for image restoration.
\newblock In {\em Proc. Int. Conf. Learn. Representations (ICLR)},
  2019.

\bibitem{irani}
M.~Zontak and M.~Irani.
\newblock Internal statistics of a single natural image.
\newblock In {\em Proc. Conf. Comput. Vis. Pattern Recognit. (CVPR)}, pp. 977--984, 2011.

\bibitem{EPLL}
D.~Zoran and Y.~Weiss.
\newblock From learning models of natural image patches to whole image
  restoration.
\newblock In {\em Proc. Int. Conf. Comput. Vis. (ICCV)}, pp.
  479--486, 2011.

\end{thebibliography}

